LocalSR: Image Super-Resolution in Local Region

Standard single-image super-resolution (SR) upsamples and restores entire images. Yet several real-world applications require higher resolutions only in specific regions, such as license plates or faces, making the super-resolution of the entire image, along with the associated memory and computational cost, unnecessary. We propose a novel task, called LocalSR, to restore only local regions of the low-resolution image. For this problem setting, we propose a context-based local super-resolution (CLSR) to super-resolve only specified regions of interest (ROI) while leveraging the entire image as context. Our method uses three parallel processing modules: a base module for super-resolving the ROI, a global context module for gathering helpful features from across the image, and a proximity integration module for concentrating on areas surrounding the ROI, progressively propagating features from distant pixels to the target region. Experimental results indicate that our approach, with its reduced low complexity, outperforms variants that focus exclusively on the ROI.

==> sec/tables/abs_context_size_train.tex <==
% swinir_context5_lightweight_lp_x2
% swinir_context5_p2_lightweight_lp_x2
% swinir_context5_p3_lightweight_lp_x2
% swinir_context5_p4_lightweight_lp_x2
% egrep 'border=0' work_dirs/super_resolution/swinir_lightweight_x2/results/500000/test_with_roi_ps24_impatch_fmstandard/test.log
% egrep -R '\[Manga109\] \[border=0\]' work_dirs/super_resolution/swinir_context5{,_p2,_p3,_p4}_lightweight_lp_x2/results/100000/test_with_roi_ps24_impatchpad18_fmfullimagev2/test.log
\begin{table}[t!]
  % \small
  \centering
  \setlength{\tabcolsep}{5pt}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{c|ccccc}
    \toprule
    % \multicolumn{2}{c|}{Context size}  & Baseline & 48 & 54 & 60 & 66 \\
    Context size  & Baseline & 48 & 54 & 60 & 66 \\
    \midrule
    PSNR & 38.22 & 38.88 & 38.88 & 38.89 & 38.88\\
    SSIM & 0.9933 & 0.9937 & 0.9937 & 0.9937 & 0.9937\\
    % \midrule
    % \multirow{2}{*}{ROI+LR} & PSNR & \\
    % & SSIM & \\
    \bottomrule
  \end{tabular}
  }
  \caption{\textbf{Ablation study on Context size during training.} The \roi{} size is $48\!\times\! 48$.} \label{table:context_size_train}
  % \vspace{-0.3cm}
  % \vspace{-0.2cm}
\end{table}

==> sec/tables/abs_full_sr.tex <==
\begin{table*}[t!]
  \centering
  \setlength{\tabcolsep}{5pt}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{c|c|c|ccc|ccc|ccc|ccc}
    \toprule
     & \multirow{2}{*}{Method} & \multirow{2}{*}{Variant}  & \multicolumn{3}{c|}{BSD100} & \multicolumn{3}{c|}{Urban100} & \multicolumn{3}{c|}{Manga109} & \multicolumn{3}{c}{Test2K}   \\
     & & &   PSNR & SSIM & GFLOPs &  PSNR & SSIM & GFLOPs & PSNR & SSIM & GFLOPs & PSNR & SSIM & GFLOPs  \\
    \midrule 
    \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{CNN}}} & \multirow{2}{*}{CARN~\cite{ahn2018fast}} & \baselineTwo{} & 27.38 & 0.8854 & 35.37 & 25.29 & 0.8879 & 209.59 & 29.27 & 0.9597 & 267.23 & 27.34 & 0.8910 & 489.93 \\
 & & Ours & \color{blue}\textbf{27.39} & \color{blue}\textbf{0.8854} & 37.51 & \color{blue}\textbf{25.32} & \color{blue}\textbf{0.8883} & 221.59 & 29.24 & 0.9595 & 282.49 & \color{blue}\textbf{27.34} & 0.8909 & 517.78 \\
\cmidrule{2-15}
& \multirow{2}{*}{SRResNet~\cite{ledig2017photo}} & \baselineTwo{} & 27.63 & 0.8895 & 158.19 & 25.99 & 0.9013 & 937.44 & 30.19 & 0.9658 & 1195.23 & 27.56 & 0.8957 & 2191.26 \\
 & & Ours & 27.62 & 0.8894 & 160.61 & \color{blue}\textbf{26.03} & \color{blue}\textbf{0.9018} & 945.02 & \color{blue}\textbf{30.20} & 0.9656 & 1204.53 & \color{blue}\textbf{27.57} & \color{blue}\textbf{0.8957} & 2207.16 \\
 \cmidrule{2-15}
& \multirow{2}{*}{RCAN~\cite{zhang2018image}} & \baselineTwo{} & 27.82 & 0.8926 & 992.73 & 26.67 & 0.9126 & 5882.85 & 31.07 & 0.9707 & 7500.64 & 27.76 & 0.8991 & 13751.17 \\
& & Ours & 27.79 & 0.8924 & 1003.03 & 26.66 & 0.9124 & 5941.75 & 31.05 & 0.9706 & 7575.61 & 27.75 & 0.8990 & 13888.26 \\
\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Transformer}}} & \multirow{2}{*}{SwinIR (lw)~\cite{liang2021swinir}} & \baselineTwo{} & 27.76 & 0.8917 & 113.70 & 26.37 & 0.9082 & 673.77 & 30.79 & 0.9693 & 859.06 & 27.71 & 0.8982 & 1574.94 \\
 & & Ours & \color{blue}\textbf{27.76} & \color{blue}\textbf{0.8918} & 122.92 & \color{blue}\textbf{26.38} & \color{blue}\textbf{0.9084} & 727.48 & \color{blue}\textbf{30.80} & 0.9692 & 927.49 & \color{blue}\textbf{27.71} & \color{blue}\textbf{0.8982} & 1700.23 \\
\cmidrule{2-15}
& \multirow{2}{*}{SwinIR~\cite{liang2021swinir}} & \baselineTwo{} & 27.90 & 0.8942 & 814.40 & 26.90 & 0.9165 & 4826.06 & 31.36 & 0.9728 & 6153.23 & 27.86 & 0.9011 & 11280.91 \\
 & & Ours & \color{blue}\textbf{27.90} & \color{blue}\textbf{0.8942} & 951.20 & \color{blue}\textbf{26.91} & \color{blue}\textbf{0.9165} & 5616.35 & \color{blue}\textbf{31.36} & \color{blue}\textbf{0.9728} & 7159.71 & 27.85 & 0.9010 & 13122.69 \\
    \bottomrule
  \end{tabular}
  }
  \caption{\textbf{Comparison on different backbones with ROI size as $24\!\times\!24$.} In this experiment, our method considers the entire LR image as the ROI and the context.} \label{table:comparison_\baselineTwo{}_vs_ours_LRinput}
\end{table*}

==> sec/tables/abs_full_sr_x2.tex <==

\begin{table*}
  \centering
  \setlength{\tabcolsep}{5pt}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{c|c|c|ccc|ccc|ccc|ccc}
    \toprule
    & \multirow{2}{*}{Method} & \multirow{2}{*}{Variant}  & \multicolumn{3}{c|}{BSD100} & \multicolumn{3}{c|}{Urban100} & \multicolumn{3}{c|}{Manga109} & \multicolumn{3}{c}{Test2K}   \\
     & & &   PSNR & SSIM & GFLOPs &  PSNR & SSIM & GFLOPs & PSNR & SSIM & GFLOPs & PSNR & SSIM & GFLOPs  \\
    \midrule 
    \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{CNN}}} & \multirow{2}{*}{CARN~\cite{ahn2018fast}} & Baseline2 &31.93 &0.9556 & 24.84 & 30.80&0.9623 &147.20 & 37.29 & 0.9920 &187.68 &32.04 & 0.9608&344.08 \\
    & & Ours & 31.92& \color{blue}\textbf{0.9556}&26.98 &   \color{blue}\textbf{30.82} & \color{blue}\textbf{0.9625}& 159.20&\color{blue}\textbf{37.34}&\color{blue}\textbf{0.9920} & 202.94& \color{blue}\textbf{32.04} & \color{blue}\textbf{0.9608}&  371.94 \\
    \cmidrule{2-15} 
    & \multirow{2}{*}{SRResNet~\cite{ledig2017photo}} &  Baseline2 &32.25 &0.9576 & 92.47 & 31.97&0.9689 & 547.95& 38.34  & 0.9932 & 698.64 & 32.49 &0.9638 & 1280.84 \\
    & & Ours &32.24 &\color{blue}\textbf{0.9576} &  94.88& \color{blue}\textbf{31.99} & \color{blue}\textbf{0.9690} & 555.53& \color{blue}\textbf{38.39} & \color{blue}\textbf{0.9932}& 707.93& \color{blue}\textbf{32.50} & \color{blue}\textbf{0.9638} & 1296.73  \\
    \cmidrule{2-15} 
    & \multirow{2}{*}{RCAN~\cite{zhang2018image}} &  Baseline2 &32.42 &0.9587 &954.68 &32.94 & 0.9735& 5657.38 & 39.20 & 0.9940 & 7213.16 & 32.83 & 0.9657 & 13224.14 \\
    & & Ours &\color{blue}\textbf{32.42} &\color{blue}\textbf{0.9588} & 964.95 & \color{blue}\textbf{32.98} &\color{blue}\textbf{0.9736} & 5716.09 & \color{blue}\textbf{39.22} & \color{blue}\textbf{0.9940} & 7287.90 &\color{blue}\textbf{32.83}& \color{blue}\textbf{0.9658} & 13360.79   \\
    \midrule 
    \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Transformer}}} & \multirow{2}{*}{SwinIR (lw)~\cite{liang2021swinir}}  & Baseline2 & 32.36 &0.9583 &37.83 & 32.44 & 0.9715 & 448.30 & 38.87 & 0.9937 & 571.59 &  32.70 & 0.9651 & 1047.91 \\
    & & Ours  & \color{blue}\textbf{32.38} &\color{blue}\textbf{0.9584} &640.02 &\color{blue}\textbf{32.49} &\color{blue}\textbf{0.9717} & 502.02 & \color{blue}\textbf{38.91} & 0.9937 & 640.02 &\color{blue}\textbf{32.71} & \color{blue}\textbf{0.9652} &1173.20 \\
    \cmidrule{2-15}
    & \multirow{2}{*}{SwinIR~\cite{liang2021swinir}}& Baseline2 & 32.52&0.9592 &  776.35& 33.26 & 0.9751 & 4600.59 & 39.37 & 0.9942 &  5865.75 & 33.00 & 0.9668 & 10753.88\\
    & & Ours & 32.51& \color{blue}\textbf{0.9593}& 913.15 & \color{blue}\textbf{33.26} & \color{blue}\textbf{0.9752} & 5390.88 & \color{blue}\textbf{39.39} & \color{blue}\textbf{0.9942} & 6872.24 & \color{blue}\textbf{33.02}&\color{blue}\textbf{0.9669} & 12595.66\\ 
    \bottomrule
  \end{tabular}
  }
  \caption{\textbf{Comparison on different backbones with ROI size as $24\!\times\!24$.} In this experiment, our method considers the entire LR image as the ROI and the context. The scale factor is set as $2$.} \label{table:comparison_\baselineTwo{}_vs_ours_LRinput_x2}
\end{table*}


==> sec/tables/sota_24x24_x2.tex <==
\begin{table*}
  \centering
  \setlength{\tabcolsep}{5pt}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{c|c|c|ccc|ccc|ccc|ccc}
    \toprule
    & \multirow{2}{*}{Method} & \multirow{2}{*}{Variant}  & \multicolumn{3}{c|}{BSD100} & \multicolumn{3}{c|}{Urban100} & \multicolumn{3}{c|}{Manga109} & \multicolumn{3}{c}{Test2K}   \\
    & & &   PSNR & SSIM & GFLOPs &  PSNR & SSIM & GFLOPs & PSNR & SSIM & GFLOPs & PSNR & SSIM & GFLOPs  \\
    \midrule 
    \parbox[t]{2mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{CNN-based}}} & \multirow{3}{*}{CARN~\cite{ahn2018fast}} & \baselineOne{} & 31.72&0.9548 &  0.46&30.42 &0.9610 & 0.46 & 36.66 & 0.9915& 0.46 &31.83 & 0.9599 & 0.46 \\
    & & \baselineTwo{} &31.93 &0.9556 & 24.84 & 30.80&0.9623 &147.20 & 37.29 & 0.9920 &187.68 &32.04 & 0.9608&344.08 \\
    & & Ours  & 31.92&\color{blue}\textbf{0.9556} & 1.70& \color{blue}\textbf{30.81} &\color{blue}\textbf{0.9625} & 5.72 & 37.27 & 0.9919 & 7.05& \color{blue}\textbf{32.04} & \color{blue}\textbf{0.9608} & 12.18\\ 
    \cmidrule{2-15} 
    & \multirow{3}{*}{SRResNet~\cite{ledig2017photo}} & \baselineOne{} & 32.04& 0.9568& 1.71&31.54 &0.9675 & 1.71 & 37.75 & 0.9928 & 1.71 &32.26 & 0.9629& 1.71 \\
    & & \baselineTwo{} &32.25 &0.9576 & 92.47 & 31.97&0.9689 & 547.95& 38.34  & 0.9932 & 698.64 & 32.49 &0.9638 & 1280.84 \\
    & &  Ours & 32.23 & 0.9575 & 4.83 & \color{blue}\textbf{31.99} &\color{blue}\textbf{0.9690} &9.87 &\color{blue}\textbf{38.35} & \color{blue}\textbf{0.9932} & 9.97 & \color{blue}\textbf{32.50} & \color{blue}\textbf{0.9638} & 16.08 \\ 
    \cmidrule{2-15} 
    & \multirow{3}{*}{RCAN~\cite{zhang2018image}} & \baselineOne{}  &32.20& 0.9578& 17.68 &32.41 & 0.9719& 17.68 & 38.46 & 0.9935 & 17.68 & 32.58& 0.9649& 17.68 \\ 
    & & \baselineTwo{} &32.42 &0.9587 &954.68 &32.94 & 0.9735& 5657.38 & 39.20 & 0.9940 & 7213.16 & 32.83 & 0.9657 & 13224.14 \\
    & & Ours  & \color{blue}\textbf{32.43}& \color{blue}\textbf{0.9588}& 40.99&\color{blue}\textbf{32.99}& \color{blue}\textbf{0.9739} & 57.43 & 39.11 & 0.9939 & 43.56 & \color{blue}\textbf{32.86} & \color{blue}\textbf{0.9660} & 46.02\\
    \midrule    
    \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Transformer-based}}} & \multirow{3}{*}{SwinIR (lw)~\cite{liang2021swinir}}  & \baselineOne{} & 32.14&0.9574 & 1.40 & 31.95 &0.9699 & 1.40 & 38.22 & 0.9933& 1.40 & 32.43  & 0.9641& 1.40\\
    & & \baselineTwo{} & 32.36 &0.9583 &37.83 & 32.44 & 0.9715 & 448.30 & 38.87 & 0.9937 & 571.59 &  32.70 & 0.9651 & 1047.91 \\
    & & Ours  &\color{blue}\textbf{32.37} &\color{blue}\textbf{0.9584} & 9.16 & \color{blue}\textbf{32.46}	& \color{blue}\textbf{0.9715} &7.98 & \color{blue}\textbf{38.88} &\color{blue}\textbf{0.9937} & 10.42 & \color{blue}\textbf{32.70} & \color{blue}\textbf{0.9651} & 13.71\\
    \cmidrule{2-15}
    & \multirow{3}{*}{SwinIR~\cite{liang2021swinir}}& \baselineOne{}  &32.27 &0.9582 & 14.38 & 32.65& 0.9732& 14.38& 38.72 &0.9938 & 14.38 & 32.69& 0.9657&14.38  \\
    & & \baselineTwo{} & 32.52&0.9592 &  776.35& 33.26 & 0.9751 & 4600.59 & 39.37 & 0.9942 &  5865.75 & 33.00 & 0.9668 & 10753.88\\
    & &  Ours & 32.50 &\color{blue}\textbf{0.9592} & 52.40 &33.21 &0.9749 & 60.19&39.34 & \color{blue}\textbf{0.9942} & 62.77 & 32.97 &0.9667 & 55.92 \\
    \bottomrule
  \end{tabular}
  }
  \caption{\textbf{Comparison on different backbones with ROI size as $24\!\times\!24$.} The scale factor is set as $2$.} \label{table:comparison_baseline_rs24_x2}
\end{table*}

==> sec/tables/sota_48x48.tex <==
\begin{table*}[t!]
  \centering
  \setlength{\tabcolsep}{5pt}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{c|c|c|ccc|ccc|ccc|ccc}
    \toprule
    & \multirow{2}{*}{Method} & \multirow{2}{*}{Variant}  & \multicolumn{3}{c|}{BSD100} & \multicolumn{3}{c|}{Urban100} & \multicolumn{3}{c|}{Manga109} & \multicolumn{3}{c}{Test2K}   \\
    & & &   PSNR & SSIM & GFLOPs &  PSNR & SSIM & GFLOPs & PSNR & SSIM & GFLOPs & PSNR & SSIM & GFLOPs  \\
    \midrule 
    \parbox[t]{2mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{CNN-based}}} & \multirow{3}{*}{CARN~\cite{ahn2018fast}}& \baselineOne{} & 28.06 & 0.9147 & 2.62 & 25.12 & 0.9026 & 2.62 & 29.06 & 0.9663 & 2.62 & 27.34 & 0.9111 & 2.62 \\
    & & \baselineTwo{} & 28.09 & 0.9149 & 35.37 & 25.21 & 0.9035 & 209.59 & 29.27 & 0.9671 & 267.23 & 27.40 & 0.9117 & 489.93 \\
 & & Ours & 28.02 & 0.9148 & 3.66 & \color{blue}\textbf{25.26} & \color{blue}\textbf{0.9045} & 7.68 & 29.26 & \color{blue}\textbf{0.9671} & 9.00 & \color{blue}\textbf{27.40} & \color{blue}\textbf{0.9118} & 14.14 \\
\cmidrule{2-15}
& \multirow{3}{*}{SRResNet~\cite{ledig2017photo}}  & \baselineOne{} & 28.34 & 0.9180 & 11.72 & 25.82 & 0.9144 & 11.72 & 29.98 & 0.9716 & 11.72 & 27.56 & 0.9150 & 11.72 \\
& & \baselineTwo{} & 28.36 & 0.9182 & 158.19 & 25.92 & 0.9154 & 937.44 & 30.18 & 0.9722 & 1195.23 & 27.62 & 0.9156 & 2191.26 \\
 & & Ours & 28.34 & 0.9180 & 13.89 & \color{blue}\textbf{25.96} & \color{blue}\textbf{0.9160} & 17.75 & \color{blue}\textbf{30.20} & 0.9720 & 19.02 & \color{blue}\textbf{27.63} & \color{blue}\textbf{0.9157} & 23.95 \\
\cmidrule{2-15}
& \multirow{3}{*}{RCAN~\cite{zhang2018image}} & \baselineOne{} & 28.53 & 0.9207 & 73.54 & 26.49 & 0.9248 & 73.54 & 30.80 & 0.9756 & 73.54 & 27.76 & 0.9180 & 73.54 \\
& & \baselineTwo{} & 28.55 & 0.9208 & 992.73 & 26.61 & 0.9259 & 5882.85 & 31.07 & 0.9764 & 7500.64 & 27.82 & 0.9186 & 13751.17 \\
 & & Ours & 28.51 & 0.9206 & 75.09 & 26.60 & 0.9257 & 77.18 & 31.03 & 0.9763 & 77.87 & 27.81 & 0.9185 & 80.53 \\
\midrule
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Transformer-based}}} & \multirow{3}{*}{SwinIR (lw)~\cite{liang2021swinir}}& \baselineOne{} & 28.47 & 0.9200 & 8.42 & 26.19 & 0.9204 & 8.42 & 30.54 & 0.9745 & 8.42 & 27.70 & 0.9170 & 8.42 \\
& & \baselineTwo{} & 28.49 & 0.9203 & 113.70 & 26.31 & 0.9217 & 673.77 & 30.79 & 0.9752 & 859.06 & 27.77 & 0.9177 & 1574.94 \\
 & & Ours & 28.48 & \color{blue}\textbf{0.9203} & 9.96 & \color{blue}\textbf{26.32} & \color{blue}\textbf{0.9219} & 13.52 & 30.76 & 0.9751 & 14.70 & \color{blue}\textbf{27.77} & \color{blue}\textbf{0.9177} & 19.25 \\
\cmidrule{2-15}
& \multirow{3}{*}{SwinIR~\cite{liang2021swinir}}& \baselineOne{} & 28.60 & 0.9220 & 60.33 & 26.67 & 0.9274 & 60.33 & 31.08 & 0.9774 & 60.33 & 27.84 & 0.9193 & 60.33 \\
& & \baselineTwo{} & 28.62 & 0.9222 & 814.40 & 26.85 & 0.9292 & 4826.06 & 31.36 & 0.9782 & 6153.23 & 27.92 & 0.9202 & 11280.91 \\
 & & Ours & 28.60 & 0.9220 & 75.76 & 26.82 & 0.9290 & 83.55 & 31.32 & 0.9781 & 86.13 & 27.91 & 0.9200 & 96.09 \\
    \bottomrule
  \end{tabular}
  }
  \caption{\textbf{Comparison on different backbones with \roi{} size as $48\!\times\! 48$.} The performance gap between ours and `\baselineTwo{}' narrows as the larger ROI size diminishes the relative impact of the context on the ROI restoration.} \label{table:comparison_baseline_rs48_x4}
\end{table*}

